A Deep Neural Network for Chinese Zero Pronoun Resolution

Existing approaches for Chinese zero pronoun resolution overlook semantic information. This is because zero pronouns have no descriptive information, which results in difficulty in explicitly capturing their semantic similarities with antecedents. Moreover, when dealing with candidate antecedents, traditional systems simply take advantage of the local information of a single candidate antecedent while failing to consider the underlying information provided by the other candidates from a global perspective. To address these weaknesses, we propose a novel zero pronoun-specific neural network, which is capable of representing zero pronouns by utilizing the contextual information at the semantic level. In addition, when dealing with candidate antecedents, a two-level candidate encoder is employed to explicitly capture both the local and global information of candidate antecedents. We conduct experiments on the Chinese portion of the OntoNotes 5.0 corpus. Experimental results show that our approach substantially outperforms the state-of-the-art method in various experimental settings.

==> reference <==
@inproceedings{mikolov2013distributed,
  title={Distributed representations of words and phrases and their compositionality},
  author={Mikolov, Tomas and Sutskever, Ilya and Chen, Kai and Corrado, Greg S and Dean, Jeff},
  booktitle={Advances in neural information processing systems},
  pages={3111--3119},
  year={2013}
}
@inproceedings{chen2014chinese,
  title={Chinese Overt Pronoun Resolution: A Bilingual Approach.},
  author={Chen, Chen and Ng, Vincent},
  booktitle={AAAI},
  pages={1615--1621},
  year={2014}
}
@article{luong2016achieving,
  title={Achieving open vocabulary neural machine translation with hybrid word-character models},
  author={Luong, Minh-Thang and Manning, Christopher D},
  journal={arXiv preprint arXiv:1604.00788},
  year={2016}
}
@inproceedings{nair2010rectified,
  title={Rectified linear units improve restricted boltzmann machines},
  author={Nair, Vinod and Hinton, Geoffrey E},
  booktitle={Proceedings of the 27th international conference on machine learning (ICML-10)},
  pages={807--814},
  year={2010}
}
@article{hobbs1978resolving,
  title={Resolving pronoun references},
  author={Hobbs, Jerry R},
  journal={Lingua},
  volume={44},
  number={4},
  pages={311--338},
  year={1978},
  publisher={Elsevier}
}
@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press}
}


@article{elman1991distributed,
  title={Distributed representations, simple recurrent networks, and grammatical structure},
  author={Elman, Jeffrey L},
  journal={Machine learning},
  volume={7},
  number={2-3},
  pages={195--225},
  year={1991},
  publisher={Springer}
}

@inproceedings{mitkov1995anaphora,
  title={Anaphora Resolution in Machine Translation},
  author={Mitkov, Ruslan and others},
  booktitle={Proceedings of the Sixth International conference on Theoretical and Methodological issues in Machine Translation},
  year={1995},
  organization={Citeseer}
}

@article{kim2000,
  title={Subject/object drop in the acquisition of Korean: A cross-linguistic comparison},
  author={Kim, Young-Joo},
  journal={Journal of East Asian Linguistics},
  volume={9},
  number={4},
  pages={325--351},
  year={2000},
  publisher={Springer}
}
@inproceedings{ferrandez2000,
  title={A computational approach to zero-pronouns in Spanish},
  author={Ferr{\'a}ndez, Antonio and Peral, Jes{\'u}s},
  booktitle={Proceedings of the 38th Annual Meeting on Association for Computational Linguistics},
  pages={166--172},
  year={2000},
  organization={Association for Computational Linguistics}
}

@article{bengio2003,
  title={A Neural probabilistic language model},
  author={Bengio, Yoshua and Ducharme, Rejean and Vincent, Pascal},
  journal={Journal of Machine Learning Research},
  volume={3},
  pages={1137--1155},
  year={2003}
}


@inproceedings{iida2006,
  title={Exploiting syntactic patterns as clues in zero-anaphora resolution},
  author={Iida, Ryu and Inui, Kentaro and Matsumoto, Yuji},
  booktitle={Proceedings of the 21st International Conference on Computational Linguistics and the 44th annual meeting of the Association for Computational Linguistics},
  pages={625--632},
  year={2006},
  organization={Association for Computational Linguistics}
}
@article{converse2006,
  title={Pronominal anaphora resolution in Chinese},
  author={Converse, Susan P},
  year={2006}
}
@inproceedings{zhao2007,
  title={Identification and Resolution of Chinese Zero Pronouns: A Machine Learning Approach.},
  author={Zhao, Shanheng and Ng, Hwee Tou},
  booktitle={EMNLP-CoNLL},
  volume={2007},
  pages={541--550},
  year={2007}
}
@inproceedings{mikolov2010,
  title={Recurrent neural network based language model.},
  author={Mikolov, Tomas and Karafi{\'a}t, Martin and Burget, Lukas and Cernock{\`y}, Jan and Khudanpur, Sanjeev},
  booktitle={INTERSPEECH 2010, 11th Annual Conference of the International Speech Communication Association, Makuhari, Chiba, Japan, September 26-30, 2010},
  pages={1045--1048},
  year={2010}
}
@inproceedings{kong2010,
  title={A tree kernel-based unified framework for Chinese zero anaphora resolution},
  author={Kong, Fang and Zhou, Guodong},
  booktitle={Proceedings of the 2010 Conference on Empirical Methods in Natural Language Processing},
  pages={882--891},
  year={2010},
  organization={Association for Computational Linguistics}
}
@inproceedings{sasano2011,
  title={A Discriminative Approach to Japanese Zero Anaphora Resolution with Large-scale Lexicalized Case Frames.},
  author={Sasano, Ryohei and Kurohashi, Sadao},
  booktitle={IJCNLP},
  pages={758--766},
  year={2011}
}
@inproceedings{chen2013,
  title={Chinese Zero Pronoun Resolution: Some Recent Advances.},
  author={Chen, Chen and Ng, Vincent},
  booktitle={EMNLP},
  pages={1360--1365},
  year={2013}
}

@inproceedings{chen2014,
  title={Chinese Zero Pronoun Resolution: An Unsupervised Approach Combining Ranking and Integer Linear Programming},
  author={Chen, Chen and Ng, Vincent},
  booktitle={Twenty-Eighth AAAI Conference on Artificial Intelligence},
  year={2014}
}
@inproceedings{chen2015,
  title={Chinese zero pronoun resolution: A joint unsupervised discourse-aware model rivaling state-of-the-art resolvers},
  author={Chen, Chen and Ng, Vincent},
  booktitle={Proceedings of the 53rd Annual Meeting of the ACL and the 7th International Joint Conference on Natural Language Processing (Volume 2: Short Papers)},
  pages={320},
  year={2015}
}
@inproceedings{chen2016,
  title={Chinese Zero Pronoun Resolution with Deep Neural Networks},
  author={Chen, Chen and Ng, Vincent},
  booktitle={Proceedings of the 54rd Annual Meeting of the ACL},
  year={2016}
}
@inproceedings{ng2007semantic,
  title={Semantic class induction and coreference resolution},
  author={Ng, Vincent},
  booktitle={AcL},
  pages={536--543},
  year={2007}
}

@phdthesis{han2006korean,
  title={Korean zero pronouns: analysis and resolution},
  author={Han, Na-Rae},
  year={2006},
  school={Citeseer}
}
@inproceedings{isozaki2003japanese,
  title={Japanese zero pronoun resolution based on ranking rules and machine learning},
  author={Isozaki, Hideki and Hirao, Tsutomu},
  booktitle={Proceedings of the 2003 conference on Empirical methods in natural language processing},
  pages={184--191},
  year={2003},
  organization={Association for Computational Linguistics}
}

@article{iida2007zero,
  title={Zero-anaphora resolution by learning rich syntactic pattern features},
  author={Iida, Ryu and Inui, Kentaro and Matsumoto, Yuji},
  journal={ACM Transactions on Asian Language Information Processing (TALIP)},
  volume={6},
  number={4},
  pages={1},
  year={2007},
  publisher={ACM}
}
@inproceedings{iida2011cross,
  title={A cross-lingual ILP solution to zero anaphora resolution},
  author={Iida, Ryu and Poesio, Massimo},
  booktitle={Proceedings of the 49th Annual Meeting of the Association for Computational Linguistics: Human Language Technologies-Volume 1},
  pages={804--813},
  year={2011},
  organization={Association for Computational Linguistics}
}
@inproceedings{sasano2008fully,
  title={A fully-lexicalized probabilistic model for japanese zero anaphora resolution},
  author={Sasano, Ryohei and Kawahara, Daisuke and Kurohashi, Sadao},
  booktitle={Proceedings of the 22nd International Conference on Computational Linguistics-Volume 1},
  pages={769--776},
  year={2008},
  organization={Association for Computational Linguistics}
}
@inproceedings{imamura2009discriminative,
  title={Discriminative approach to predicate-argument structure analysis with zero-anaphora resolution},
  author={Imamura, Kenji and Saito, Kuniko and Izumi, Tomoko},
  booktitle={Proceedings of the ACL-IJCNLP 2009 Conference Short Papers},
  pages={85--88},
  year={2009},
  organization={Association for Computational Linguistics}
}
@inproceedings{hayashibe2011japanese,
  title={Japanese Predicate Argument Structure Analysis Exploiting Argument Position and Type.},
  author={Hayashibe, Yuta and Komachi, Mamoru and Matsumoto, Yuji},
  booktitle={IJCNLP},
  pages={201--209},
  year={2011}
}
@article{iida2015intra,
  title={Intra-sentential zero anaphora resolution using subject sharing recognition},
  author={Iida, Ryu and Torisawa, Kentaro and Hashimoto, Chikara and Oh, Jong-Hoon and Kloetzer, Julien},
  journal={Proceedings of EMNLP’15},
  pages={2179--2189},
  year={2015},
  publisher={Citeseer}
}
@inproceedings{wiseman2015learning,
  title={Learning anaphoricity and antecedent ranking features for coreference resolution},
  author={Wiseman, Sam Joshua and Rush, Alexander Matthew and Shieber, Stuart Merrill and Weston, Jason},
  year={2015},
  organization={Association for Computational Linguistics}
}
@inproceedings{clark2016improving,
 author = {Clark, Kevin and Manning, Christopher D.},
 booktitle = {Association for Computational Linguistics (ACL)},
 title = {Improving Coreference Resolution by Learning Entity-Level Distributed Representations},
 year = {2016}
}
@article{clark2016deep,
  title={Deep reinforcement learning for mention-ranking coreference models},
  author={Clark, Kevin and Manning, Christopher D},
  journal={arXiv preprint arXiv:1609.08667},
  year={2016}
}
@article{soon2001machine,
  title={A machine learning approach to coreference resolution of noun phrases},
  author={Soon, Wee Meng and Ng, Hwee Tou and Lim, Daniel Chung Yong},
  journal={Computational linguistics},
  volume={27},
  number={4},
  pages={521--544},
  year={2001},
  publisher={MIT Press}
}
@incollection{ng2016advanced,
  title={Advanced Machine Learning Models for Coreference Resolution},
  author={Ng, Vincent},
  booktitle={Anaphora Resolution},
  pages={283--313},
  year={2016},
  publisher={Springer}
}
@inproceedings{guodong2008context,
  title={Context-sensitive convolution tree kernel for pronoun resolution},
  author={Guodong, Zhou and Fang, Kong and Qiaoming, Zhu},
  year={2008},
  booktitle = {Proceedings of the 3rd International Joint Conference on Natural Language Processing}

}
